Multidimensional Resource Fragmentation-Aware Virtual Network Embedding in MEC Systems Interconnected by Metro Optical Networks

The increasing demand for diverse emerging applications has resulted in the interconnection of multi-access edge computing (MEC) systems via metro optical networks. To cater to these diverse applications, network slicing has become a popular tool for creating specialized virtual networks. However, resource fragmentation caused by uneven utilization of multidimensional resources can lead to reduced utilization of limited edge resources. To tackle this issue, this paper focuses on addressing the multidimensional resource fragmentation problem in virtual network embedding (VNE) in MEC systems with the aim of maximizing the profit of an infrastructure provider (InP). The VNE problem in MEC systems is transformed into a bilevel optimization problem, taking into account the interdependence between virtual node embedding (VNoE) and virtual link embedding (VLiE). To solve this problem, we propose a nested bilevel optimization approach named BiVNE. The VNoE is solved using the ant colony system (ACS) in the upper level, while the VLiE is solved using a combination of a shortest path algorithm and an exact-fit spectrum slot allocation method in the lower level. Evaluation results show that the BiVNE algorithm can effectively enhance the profit of the InP by increasing the acceptance ratio and avoiding resource fragmentation simultaneously.

==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf

